SwitchDelta: Asynchronous Metadata Updating for Distributed Storage with In-Network Data Visibility

Distributed storage systems typically maintain strong consistency between data nodes and metadata nodes by adopting ordered writes: 1) first installing data; 2) then updating metadata to make data visible.We propose SwitchDelta to accelerate ordered writes by moving metadata updates out of the critical path. It buffers in-flight metadata updates in programmable switches to enable data visibility in the network and retain strong consistency. SwitchDelta uses a best-effort data plane design to overcome the resource limitation of switches and designs a novel metadata update protocol to exploit the benefits of in-network data visibility. We evaluate SwitchDelta in three distributed in-memory storage systems: log-structured key-value stores, file systems, and secondary indexes. The evaluation shows that SwitchDelta reduces the latency of write operations by up to 52.4% and boosts the throughput by up to 126.9% under write-heavy workloads.

==> sec/table1.tex <==
\begin{table}[!h]
\begin{tabular}{|l|l|l|l|}
\hline
            & KV    & SI                &    ?   \\ \hline
Data        & Log   & Primary Index     &       \\ \hline
Metadata    & Index & Secondary Index   &       \\ \hline
Ordering    &  &  &       \\ \hline
\end{tabular}
\end{table}
